Sketching as a Tool for Understanding and Accelerating Self-attention for Long Sequences

Transformer-based models are not efficient in processing long sequences due to the quadratic space and time complexity of the self-attention modules. To address this limitation, Linformer and Informer are proposed to reduce the quadratic complexity to linear (modulo logarithmic factors) via low-dimensional projection and row selection respectively. These two models are intrinsically connected, and to understand their connection, we introduce a theoretical framework of matrix sketching. Based on the theoretical analysis, we propose Skeinformer to accelerate self-attention and further improve the accuracy of matrix approximation to self-attention with three carefully designed components: column sampling, adaptive row normalization and pilot sampling reutilization. Experiments on the Long Range Arena (LRA) benchmark demonstrate that our methods outperform alternatives with a consistently smaller time/space footprint.

==> algorithm/skein.tex <==
\begin{algorithm}
\SetAlgoLined
\KwIn{query matrix $\mtx{Q}$, key matrix $\mtx{K}$, value matrix $\mtx{V}$ (all are $n$-by-$p$), and sub-sample size $d$}
\KwOut{An $n$-by-$p$ matrix $\mtx{R}$}
 % Initialize the matrix $\mtx{R} = 0 \in \mb R^{n \times d}$\; 
 Run Algorithm~\ref{Alg:incomplete} to obtain the output $\mtx{R}$ and the intermediate variable $\mtx{B}_J$ in Line~3\;
 Compute $\mtx{B}_J \mtx{V}$ and assign it to the corresponding rows of $\mtx{R}$\;
 \caption{Skeinformer+.}
\label{Alg:skein}
\end{algorithm}


==> figures/lra.tex <==
\begin{figure}[htbp]
\centering
\includegraphics[width=0.9\linewidth]{figures/LRASVD.png}
\caption{
Singular value distribution of attention output from the second layer of standard transformer. 
Results are averaged across one batch from test set.
---conclusion from this fig --- }
\label{fig:lra}
\end{figure}

==> figures/norm_all.tex <==
\begin{figure}[htbp]
\centering
\includegraphics[width=0.95\linewidth]{figures/skein_norm_all.png}
\caption{
Spectral norm results with the sequence length of 1024 and 4096.
% under different $W_Q, W_K, W_V$ settings, either from initialized or pretrained BERT models. 
Y axis: Lower percentage score means better approximation. 
X axis: Higher number of feature means larger computation cost.}
\label{fig:norm_all}
\end{figure}

==> figures/valloss.tex <==
\begin{figure*}[htbp]
\centering

\includegraphics[width=1.0\linewidth]{figures/aaai_baseline_loss7.png}
\caption{Validation loss changes with regards to total training time (s). 
% Our proposed variants and Informer can efficiently converge to the long-time limit, while Linformer fails to attain a stationary distribution as good as the original softmax.
}
\label{fig:valloss}
\end{figure*}

==> tables/lra_results.tex <==
\begin{table*}[h]
\small
\centering
\begin{tabular}{l|c|c|c|c|c|c|c|c|c|c|c|c|c}
\hline
Models & \multicolumn{3}{c|}{Text (4k)} & \multicolumn{3}{c|}{ListOps (2k)} & \multicolumn{3}{c|}{Retrieval (4k)}  & \multicolumn{3}{c|}{Pathfinder (1k)} & \textbf{Avg} \\
\cline{2-14}
 & acc  & step & time  & acc  & step & time    & acc  & step & time    & acc  & step & time & acc  \\
\hline
Standard &57.69&	11&	3038&		38.15&	9&	1338&		80.10&	20&	3196&		73.59&	21&	835 & 62.38 \\
\hline
Big Bird  & 61.91 & 	6 & 	1235 & 		38.86 & 	9 & 	1037 & 		79.73 & 	15 & 	1304 & 		71.75 & 	17 & 	1070 & 63.06\\
Linformer & 58.52 & 	7 & 	474 & 		37.97 & 	11 & 	375 & 		77.40 & 	23 & 	485 & 		55.57 & 	7 & 	414  & 57.36 \\
Informer  & 61.55  & 	8  & 	1988  & 		38.43  & 	10  & 	1313  & 	80.88  & 	25  & 	2191  & 		59.34  & 	9  & 	1569 & 60.05\\
Performer & 57.67 & 	30 & 	158 & 		37.70 & 	10 & 	558 & 		75.69 & 	13 & 	750	 & 	56.50 & 	9 & 	624 & 56.89\\
Nystr\"omformer & 60.91 & 	12 & 	731	 & 	37.76 & 	10 & 	737	 & 	79.87 & 	17 & 	801	 & 	72.53 & 	23 & 	1175 & 62.77\\

\hline
Skeinformer & 62.39 & 	7 & 	429	 & 	38.12 & 	6 & 	439	 & 	79.88 & 	22 & 	521	 & 	71.53 & 	17 & 	425 & 	62.98\\
\textbf{Skeinformer+}  & 62.47 & 	6 & 	576	 & 	38.73 & 	7 & 	580	 & 	80.42 & 	20 & 	636	 & 	71.51 & 	18 & 	555	 & 	\textbf{63.28}\\

\hline
\end{tabular}
\caption{
Classification accuracy (\%) on test sets, training steps (k) and training time (s) per thousand steps on LRA benchmark. 
In general our proposed methods achieve competitive or even better performance than standard full attention with much less training time. 
For example, Skeinformer+ has $4.78\%$ accuracy improvement and nearly $10\times$ speed-up on text classification over standard method.
Comparing to other attention approximation methods, Skeinformer+ has the best overall performance.
}
\label{table:lra}
\end{table*}
%%% EMNLP
